Depth Is All You Need for Monocular 3D Detection

A key contributor to recent progress in 3D detection from single images is monocular depth estimation. Existing methods focus on how to leverage depth explicitly, by generating pseudo-pointclouds or providing attention cues for image features. More recent works leverage depth prediction as a pretraining task and fine-tune the depth representation while training it for 3D detection. However, the adaptation is insufficient and is limited in scale by manual labels. In this work, we propose to further align depth representation with the target domain in unsupervised fashions. Our methods leverage commonly available LiDAR or RGB videos during training time to fine-tune the depth representation, which leads to improved 3D detectors. Especially when using RGB videos, we show that our two-stage training by first generating pseudo-depth labels is critical because of the inconsistency in loss distribution between the two tasks. With either type of reference data, our multi-task learning approach improves over the state of the art on both KITTI and NuScenes, while matching the test-time complexity of its single task sub-network.

==> figures/network_structure.tex <==
\begin{figure*}
\centering
% \subfloat[\centering DD3D Head]{{\includegraphics[trim={10cm 0 0 0},clip,width=0.4 \linewidth]{figures/images/DD3D.png} }}%
% \subfloat[\centering DD3Dv2 Head]{{\includegraphics[trim={10cm 0 0 0},clip,width=0.4 \linewidth]{figures/images/DD3Dv2.png} }}%
\includegraphics[width=\textwidth]{figures/images/DD3Dv2-single.png}
\caption{Multi-task detection and depth estimation head. We completely remove the 2D box feature tower from DD3D to decrease the overhead from depth to 3D detection. We add a seperate depth tower for dense depth estimation.}
\label{fig:architecture}
\end{figure*}

==> figures/visualization.tex <==
\begin{figure*}[h]
\centering
\subfloat{{\includegraphics[width=\textwidth]{figures/images/fig-3-gt.png} }}\\
\subfloat{{\includegraphics[width=\textwidth]{figures/images/fig-3-sup.png} }}\\
\subfloat{{\includegraphics[width=\textwidth]{figures/images/fig-3-selfsup.png} }}\\
\caption{\textbf{Visualization of detectors.} The \textbf{top} row shows the ground-truth 3D boxes on 4 images in nuScenes \emph{validation} split. The \textbf{middle} and \textbf{bottom} rows shows the detection from our approaches, multi-task training using point-cloud data and our two-stage pseudo-labels approach, respectively. In the top-down view on the upper-right corners, we show the ground-truth (\textbf{green}) overlaid with the detection (\textbf{red}).}
\label{fig:visualization}
\end{figure*}

==> sections/8_limitation.tex <==
\section{LIMITATIONS}
Our two-stage pseudo-depth approach addresses the impractical assumption that point-cloud data is only be available at training time, which is a limitation of most related methods. However, our method is still limited in that it utilizes available video frames only during training, and operates in a monocular setting at test time. It is plausible to extend our work to use similar geometric constraints at test time, to further push the limits of detection accuracy.

==> tables/complexity.tex <==
\begin{table}[h]
\centering
{
\begin{tabular}{l|c|c}
Methods & params. & runtime [ms/sample] \\
\midrule
% 78622283, 2.1fps
DETR3D & 75.0M  & 476 \\
% 81664736 3.5fps
PETR-e & 77.9M  & 285 \\
\midrule
DD3Dv2 & 78.1M  & x.xx \\ 
\end{tabular}

\vspace{1em}

\caption{\textbf{Comparision with DD3D.} We evaluate the \emph{original} DD3D with DD3Dv2 to ablate the effect of the modifications proposed in Sec.~\ref{sec:dd3dv2}.}
\label{tab:orig_dd3d}
}
\vspace{-5mm}
\end{table}

==> tables/depth-source.tex <==
\begin{table}[t!]
\centering
{
\rowcolors{2}{lightgray}{white}
\begin{tabular}{c|c|c|c|c|c}
source of depth& Depth Loss &source $abs\_rel$ & final $abs\_rel$ & mAP[$\%$]$\uparrow$ \\

\midrule
None & -&- & - & $35.8$ \\%https://wandb.ai/tri/multitask/runs/21sj56jo
\midrule
 \multicolumn{5}{c}{Direct Supervision in Multitask} \\
 \midrule
%https://wandb.ai/tri/multitask/runs/1b62oxvo
Nuscene Lidar & L1&- & - & $39.1$ \\
Nuscene Selfsup. & SSIM&- & - & $36.4$ \\ %https://wandb.ai/tri/multitask/runs/domqet7u
$+$ remove moving obj.  & SSIM&- & - & $36.2$ \\ %https://wandb.ai/tri/multitask/runs/1aqs4c77
\midrule
 \multicolumn{5}{c}{Distillation} \\
 \midrule
IODA Pre. & L1& - & - & - \\
Nuscene sup. & L1&- & - & - \\
%https://wandb.ai/tri/multitask/runs/thcuygv5
Nuscene 3D obj~\cite{zhang2022monodetr} & L1&- & - & - \\
\midrule
Nuscene self-sup &L1& - & - & $37.7$ \\%https://wandb.ai/tri/multitask/runs/2yhew5a2
$+$ remove moving obj. &L1& - & - & - \\
\bottomrule
\end{tabular}
\caption{Depth source.}
}
\end{table}

==> tables/depth-supervision-objective.tex <==
\begin{table}[t!]
\centering
{
\rowcolors{2}{lightgray}{white}
\begin{tabular}{c|c|c}
Supervised loss &  $abs\_rel$ & mAP[$\%$]$\uparrow$ \\

\midrule
L1 & - & -  \\
Berhu & - & -  \\
Self-sup. & - & -  \\
\bottomrule
\end{tabular}
\caption{Supervision Loss}
}
\end{table}

==> tables/kitti_ablation.tex <==
\begin{table}[h]
\centering
{
\begin{tabular}{l|c|c|c}
\thead{Adaptation \\ strategies} & \multicolumn{3}{c}{\thead{Detection Accuracy \\ BEV AP $\uparrow$ \darkgray{(Box AP [$\%$]$\uparrow$)}} }\\
& Car & Ped. & Cyc.\\
\midrule
% https://wandb.ai/tri/multitask/runs/2x2fl267
\small{\thead{DD3Dv2 \\ \small{(no-depth)}}} & 33.5 \darkgray{(24.4)}&13.2 \darkgray{(11.0)}&4.1 \darkgray{(3.7)} \\
\midrule
\multicolumn{4}{c}{\small{\textbf{Multi-task} (single stage)}} \\
\midrule
% https://wandb.ai/tri/multitask/runs/141h42xe
Supervised  & 
34.0 \darkgray{(25.0)}&
15.3 \darkgray{(12.9)}&
7.4 \darkgray{(6.3)} \\
%\midrule
%\multicolumn{4}{c}{\small{\textbf{Pseudo-labels $\rightarrow$ Multi-task}}} \\
%\midrule
%Self-supervised & xx.x \darkgray{(xx.x)}&xx.x \darkgray{(xx.x)}&xx.x \darkgray{(xx.x)} \\ 
% TODO: paste a wandb link
\end{tabular}

\vspace{1em}

\caption{\textbf{Ablation on KITTI.} We present an abridged version of Table~\ref{tab:ablation}, but now on KITTI 3D dataset.}
\label{tab:kitti_ablation}
}
\vspace{-5mm}
\end{table}

==> tables/nuscenes-weight-loss.tex <==

% \begin{table}[t!]
% \centering
% {
% \footnotesize
% \setlength{\tabcolsep}{0.4em}
% \rowcolors{2}{lightgray}{white}
% \begin{tabular}{l|c|c|c}
% \toprule
% Class & 
% PointPillars~\cite{lang2019pointpillars} &
% MonoDIS (multi)~\cite{simonelli2020disentangling} &
% FCOS-3D \\
% \midrule

% Barrier      & 39.0   & 50.0 & - \\
% Bicycle      & 1.0    & 25.0 & - \\
% Bus          & 28.0   & 15.0 & - \\
% Car          & 68.0   & 46.0 & - \\
% Constr. Veh. & 4.0    & 6.0  & - \\
% Motorcycle   & 27.0   & 30.0 & - \\
% Pedestrian   & 60.0   & 36.0 & - \\
% Traffic Cone & 31.0   & 49.0 & - \\
% Trailer      & 23.0   & 16.0 & - \\
% Truck        & 23.0   & 21.0 & - \\
% \midrule
% Mean AP [\%] $\uparrow$ & 31.0 & 30.0 & - \\


% % \bottomrule
% \end{tabular}\\\vspace{0mm}
% \caption{
% \textbf{3D detection performance on the nuScenes~\cite{caesar2020nuscenes} test set for all the classes.} We report the \textit{Average Precision} for each class, and the Mean AP over all the classes for each method.}
% \label{table:nuscenes_test_summary}
% }
% \end{table}



\begin{table}[h]
% wandb report;
\centering
{
\tiny
\footnotesize
\setlength{\tabcolsep}{0.3em}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{c|cc|c}
\toprule
Loss Weight& AP[$\%$]$\uparrow$ &  NDS$\uparrow$ & Abs. Rel $\downarrow$ \\
\midrule
0.55 &{38.0} &  {0.45}&\textbf{0.20}\\
%https://wandb.ai/tri/multitask/runs/2evxwhiv
0.45 &\textbf{39.1} &  {\textbf{0.46}}& \textbf{0.20}\\
%https://wandb.ai/tri/multitask/runs/12wsqej2
0.35 &{38.9} &  {0.45}&\textbf{0.20}\\
%https://wandb.ai/tri/multitask/runs/3v47xod0
0.25 &{38.1} &  {0.44}&\textbf{0.20}\\
%https://wandb.ai/tri/multitask/runs/1sll4iek
0.15 &{37.9} &  {0.44}&0.21\\
%https://wandb.ai/tri/multitask/runs/3aiypfed
\midrule
0 &35.8 &0.41 &-\\
%https://wandb.ai/tri/multitask/runs/3aiypfed
 \bottomrule
\end{tabular}\\\vspace{2mm}
\caption{Detection accuracy vs. depth loss weight. We fix the weight for 3D box loss to $1.0$, and search for the optimal value for depth loss in case of our multi-task training using point-cloud.}
\label{table:nuscenes-loss-weight}
}
\end{table}


==> tables/nuscenes_detailed.tex <==

\begin{table*}[]
\centering
{
\setlength{\tabcolsep}{4.5pt}
\footnotesize
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
& \multicolumn{4}{c}{Car [\%] $\uparrow$} & \multicolumn{4}{c}{Pedestrian [\%] $\uparrow$} &  \multicolumn{4}{c}{Bicycle [\%] $\uparrow$} \\

\multirow{-2}{*}{Methods}& 
0.5m & 1.0m & 2.0m & 4.0m & 0.5m & 1.0m & 2.0m & 4.0m & 0.5m & 1.0m & 2.0m & 4.0m\vspace{0.5mm}\\

\midrule

% CenterNet$^*$  &
% 20.0 & 45.8 & 68.0 & 80.6 &
% 7.9 & 26.7 & 49.6 & 65.9 &
% 4.3 & 13.8 & 28.4 & 36.2 \\

% AIML-ADL$^*$ &
% 14.2 & 36.8 & 58.5 & 71.0 &
% 9.6 & 30.8 & 54.6 & 69.4 &
% 5.2 & 21.6 & 37.3 & 46.2 \\

% DHNet$^*$ &
% 15.2 & 37.9 & 59.4 & 71.5 &
% 10.5 & 31.7 & 55.7 & 69.9 &
% 5.6 & 24.2 & 38.9 & 48.0 \\

% PGDepth$^*$    &
% 17.0 & 43.6 & 67.2 & 80.3 &
% 9.1 & 31.0 & 53.9 & 69.1 &
% 7.6 & 24.1 & 40.1 & 49.2 \\
MonoDis~\cite{simonelli2019disentangling} &
10.7 &
37.5 &
{69.0} &
{85.7} &
- &
- &
- &
- &
- &
- &
- &
- \\
% MonoDis (multi)~\cite{simonelli2020disentangling} & 
% 10.6 & 36.1 & 65.0 & 80.5 &
% 6.7 & 30.0 & 48.5 & 64.7 &
% 4.4 & 17.5 & 32.8 & 43.9 \\
FCOS3D~\cite{wang2021fcos3d}    &
{15.3} & {43.8} & 68.9 & 81.7 &
{8.7} & {30.3} & {52.9} & {67.1} & 
{7.9} & {25.0} & {39.2} & {47.1} \\
PGD\cite{wang2022probabilistic}    &
{20.4} & {48.7} & 71.8 & 83.4 &
{11.6} & {35.0} & {58.0} & {71.9} & 
{9.7} & {26.2} & {40.4} & {49.1} \\
DD3D~\cite{park2021dd3d} &
{30.2} &
{59.7} &
{77.4} &
{84.1} &
{18.7} &
{42.4} &
{61.9} &
{70.2} &
{15.7}  &
{32.6} &
{45.2} &
{50.0} 
\\
DETR3D~\cite{detr3d}   &
24.1 & 56.2 & {78.1} & {86.7} &
 12.8& 37.3 & 61.6 & {74.3} & 
 10.6& 25.9 & 39.5 & 44.9 \\
\midrule
% unpublished method
BEVDet$^*$~\cite{huang2021bevdet}&
{31.6} & {62.3} & 78.7& 84.3 &
{17.8} & {37.2} & {51.2} & {58.1} & 
{13.5} & {29.0} & {36.6} & {39.1} \\
PETR$^*$~\cite{liu2022petr}     &
{29.6} & {57.8} & 78.1 & \textbf{86.8} &
{13.5} & {39.1} & {62.7} & {74.6} & 
{10.2} & {27.1} & {40.2} & {45.1} \\
\midrule
%"car": {"0.5": 0.3130879826412605, "1.0": 0.600097385413361, "2.0": 0.7806188249781087, "4.0": 0.8520682001205703},
DD3Dv2-Selsup. &{31.3} & {60.0} & {78.1} &85.2
%"pedestrian":{"0.5": 0.19124375823585954, "1.0": 0.43211403004056936, "2.0": 0.627885037024185, "4.0": 0.7299405356391677}, 
 & {19.1} & {44.2} & {62.8} & 73.0 &
%"bicycle": {"0.5": 0.17546062864084366, "1.0": 0.3353361838200302, "2.0": 0.4685883655445414, "4.0": 0.5252648363200102}, 
{17.5} & {33.5} & {46.9} & {52.5} \\
%
%"car": {"0.5": 0.3596536094332398, "1.0": 0.6307015909262296, "2.0": 0.7949206469445562, "4.0": 0.8612389284170383}, 
DD3Dv2 & \textbf{40.0} & \textbf{63.1} & \textbf{79.5} & {86.1}
%"pedestrian": {"0.5": 0.25586117613785087, "1.0": 0.4906324224874566, "2.0": 0.6662985816131062, "4.0": 0.7533312191925321},
 & \textbf{25.6} & \textbf{49.1} & \textbf{66.6} & \textbf{75.3} &
%"bicycle": {"0.5": 0.22941239538697897, "1.0": 0.40273232048042373, "2.0": 0.4965852696170633, "4.0": 0.5323647561498759},
\textbf{22.9} & \textbf{40.3} & \textbf{49.7} & \textbf{53.2}

\end{tabular}\\\vspace{0mm}
\caption{
\textbf{Detailed results on the nuScenes \textit{test} set.} We report mean AP metrics on \emph{Car}, \emph{Pedestrian}, and \emph{Bicycle} with varying thresholds on distance. The \textbf{bold} denotes the best of all.
%\textbf{DD3D detection results on the nuScenes~\cite{caesar2020nuscenes} test set:} we report detailed results on the \textit{Car}, \textit{Pedestrian} and \textit{Bicycle} classes; detailed results for the other classes can be found in the supplementary. * denotes results reported from  the nuScenes official test set that do not have an associated publication at the time of writing.
}
\label{table:nuscenes_test_detailed}
}
\end{table*}
